Optimal Non-Adaptive Cell Probe Dictionaries and Hashing

We present a simple and provably optimal non-adaptive cell probe data structure for the static dictionary problem. Our data structure supports storing a set of n key-value pairs from [u]x[u] using s words of space and answering key lookup queries in t = O(lg(u/n)/ lg(s/n)) nonadaptive probes. This generalizes a solution to the membership problem (i.e., where no values are associated with keys) due to Buhrman et al. We also present matching lower bounds for the non-adaptive static membership problem in the deterministic setting. Our lower bound implies that both our dictionary algorithm and the preceding membership algorithm are optimal, and in particular that there is an inherent complexity gap in these problems between no adaptivity and one round of adaptivity (with which hashing-based algorithms solve these problems in constant time). Using the ideas underlying our data structure, we also obtain the first implementation of a n-wise independent family of hash functions with optimal evaluation time in the cell probe model.

==> explicit-expanders.tex <==
\section{Lower Bounds and Explicit Constructions for Non-Contractive Expanders}
\label{sec:expander}

In this section, we first note that our non-explicit $(\leq n)$-non-contractive expanders are optimal for most settings of parameters.
This follows from a result of Radhakrishnan and Ta-Shma \cite{RadhakrishnanT00} who prove that any $(u,s,t)$-bipartite graph with expansion $1$ requires $d=\Omega(\log (u/n) / \log (s/n))$. 
In more detail, Theorem 1.5 (a) of \cite{RadhakrishnanT00} proves that if $G$ is a $(u,s,t)$-bipartite graph that is an $(n,\epsilon)$ disperser, then the left-degree, $t$, is $\Omega((1-\epsilon)s)$. Since a $(\leq n,1)$-non-contractive expander is also an $(n,\epsilon)$-disperser with $(1-\epsilon) = n/s$, the lower bound $t = \Omega(\log(u/n)/\log (s/n))$ follows.
Thus in order to implement our non-adaptive dictionary in the word-RAM model, we require an explicit construction of $(\leq n,1)$-bipartite expander graphs that that are essentially optimal in terms of degree.

TODO KGL: I think this is not completely solid and would degenerate to A = Omega(1).

Next we show a near converse to the above: any non-adaptive dictionary in the word-RAM model matching our parameters implies an explicit construction of near-optimal $(\leq n,1)$-bipartite expanders.
As before, $w = \Theta(\lg u)$ and $X$ denotes a subset of $U = \{0,\ldots,u-1\}$ of size $n$. We will assume $u \geq n^c$, where $c >1$. For smaller $u$, it is conceivable that optimal dictionaries may be constructed without efficient $(\leq n,1)$-bipartite expanders.

Assume that there exists a non-adaptive word-RAM dictionary for solving the membership
problem, on all subsets $X \subseteq U$ of size $n$, using $s$ memory cells and $t$ cell probes per query. 
%(As before, we assume the word size $w = \Theta(u)$).
%We will write $u=n^c$, where $c>1$, since the problem is trivial when $n=O(c)$.
Since the algorithm is non-adaptive, associated with the algorithm is a bipartite graph $G_f$ represented by the function $f: \{0,\ldots,u-1\} \times \{1,\ldots, t\} \rightarrow \{1,\ldots,s\}$
where $f(x,1),\ldots,f(x,t)$ are the indices of the $t$ memory cells that are probed on query $x \in U$.
%is assumed to be in the word-RAM model, we require that $f$ is efficiently computable.

In order to be able to answer all queries correctly, for every subset $X$ of size $n$, the algorithm needs to probe at least $\log {u \choose n}$ bits of memory. (Since otherwise, by the pigeonhole principle there would be two different sets, $X$ and $X'$ such that the algorithm would give the same answers on the query sets $\{x ~|~ x \in X\}$ and $\{x ~|~ x \in X'\}$.)
Now suppose that $A$ is the expansion factor of $G_f$, so we have $|\Gamma(X)| = An$ for all subsets $X$ of size $n$. Therefore $An$ cells are probed in total as we query every $x \in X$; since each cell contains $\log u$ bits of storage, we require:

$$An \log u \geq  \log {u \choose n} \geq \log (u/n)^n = n \log(u/n).$$

Solving for $A$ with $u=n^c$ gives $A \geq \log(u/n)/\log u = (c-1)/c = 1-\frac{1}{c}$.
Thus any non-adaptive algorithm in the word-RAM model implies an explicit construction
of a bipartite graph $G_f$ such that for every $n=u^{1/c}$, and for every subset $X$ of
left vertices of size $n$, $|\Gamma(X)| \geq 1-\frac{1}{c}$. Note that our algorithm requires expansion factor 1 on all subsets of size at most $n$ and thus the expansion factor that is implied by a word-RAM implementation is slightly smaller (and thus slightly weaker) than what our algorithm requires for large subsets. 
%However we note that our upper bound can be modified to work even if $G_f$ has
%slightly less expansion, $1-\frac{1}{c}$.
%For this improvement, we will group the $n$ elements of $X$ into
%$c$ groups, each of size $n/c$ (because a single cell contains $c \log n$ bits of memory).
% With this grouping, we modify the preprocessing step
%to map an entire group into a single cell, which
%effectively lowers the required expansion to $1-\frac{1}{c}$.




